A Spatial Array for Spectrally Agile Wireless Processing

Massive MIMO is a cornerstone of next-generation wireless communication, offering significant gains in capacity, reliability, and energy efficiency. However, to meet emerging demands such as high-frequency operation, wide bandwidths, co-existence, integrated sensing, and resilience to dynamic interference, future systems must exhibit both scalability and spectral agility. These requirements place increasing pressure on the underlying processing hardware to be both efficient and reconfigurable. This paper proposes a custom-designed spatial array architecture that serves as a reconfigurable, general-purpose core optimized for a class of wireless kernels that commonly arise in diverse communications and sensing tasks. The proposed spatial array is evaluated against specialized cores for each kernel using High-Level Synthesis (HLS). Both the reconfigurable and specialized designs are synthesized in a 32 nm process to assess latency, throughput, area, and power in realistic processes. The results identify conditions under which general-purpose systolic architectures can approach the efficiency of specialized cores, thereby paving the way toward more scalable and agile systems.

==> defs/macros.tex <==
\ProvidesPackage{FletcherGroupMacros}[2020/10/04 v1.0 Macros for Fletcher group papers]

\RequirePackage{xcolor,bm,setspace}
\RequirePackage{mathrsfs}
\RequirePackage{amsmath}
\RequirePackage{amsfonts}
% \RequirePackage{amsthm}
\RequirePackage{enumitem}


\providecommand{\loss}{\mc{L}}
\providecommand{\reg}{\mc{R}}

\def\ts{{\rm ts}}
\def\tr{{\rm tr}}
% \providecommand{\innerx}[1]{\left<#1\right>_x}
% \providecommand{\innerz}[1]{\left<#1\right>_z}

% coloring
%\usepackage[normalem]{ulem} % provides strikeout command \sout
\newcommand{\textr}[1]{\textcolor{red}{#1}}
\newcommand{\textg}[1]{\textcolor{green}{#1}}
\newcommand{\textb}[1]{\textcolor{blue}{#1}}


\renewcommand{\tilde}{\widetilde}
\renewcommand{\hat}{\widehat}
\renewcommand{\bf}{\boldsymbol}
\def\del{\partial}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
\def\beqan{\begin{eqnarray*}}
\def\eeqan{\end{eqnarray*}}
\def\nn{\nonumber}
\def\half{{\tfrac{1}{2}}}
\def\Half{{\frac{1}{2}}}
\def\N{{\mathbb{N}}}
\def\Z{{\mathbb{Z}}}
\def\Q{{\mathbb{Q}}}
\def\R{{\mathbb{R}}}
\def\C{{\mathbb{C}}}
\def\Gbar{\wb G}
\DeclareMathOperator*{\binomial}{binomial}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\prox}{prox} %
\DeclareMathOperator*{\sign}{sign}
\def \cov{\mathrm{cov}}
\def\mp{{\rm{mp}}}
\def\var{\mathrm{var}}
\def\x{\bm{x}}
\def\limn{\lim_{n \rightarrow \infty}}
\def\liminfn{\liminf_{n \rightarrow \infty}}
\def\limsupn{\limsup_{n \rightarrow \infty}}
\def\MID{\,|\,}
\def\MIDD{\,;\,}
\newcommand{\Wass}{\stackrel{(2)}{\Rightarrow}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\def\inv{^{-1}}
\def\slam{s,\lambda}

% \newtheorem{proposition}{Proposition}
%\newtheorem{claim}{Claim}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \theoremstyle{definition}
% \newtheorem{example}{Example}
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{remark}{Remark}
\def\qed{\mbox{} \hfill $\Box$}
\setlength{\unitlength}{1mm}

\def\bhat{\wh{b}}
\def\bbar{\overline{b}}
\def\ehat{\wh{e}}
\def\fhat{\wh{f}}
\def\gtilde{\tilde{g}}
\def\phat{\wh{p}}
\def\qhat{\wh{q}}
\def\rhat{\wh{r}}
\def\shat{\wh{s}}
\def\uhat{\wh{u}}
\def\vhat{\wh{v}}
\def\xhat{\wh{\x}}
\def\xbar{\overline{x}}
\def\zhat{\widehat{z}}
\def\what{\widehat{w}}
\def\zbar{\overline{z}}
\def\la{\leftarrow}
\def\ra{\rightarrow}
\def\MSE{\mbox{\small \sffamily MSE}}
\def\SNR{\mbox{\small \sffamily SNR}}
\def\SINR{\mbox{\small \sffamily SINR}}
\def\arr{\rightarrow}
\def\Exp{\mathbb{E}\,}
\def\Prob{\mathbb{P}}
\def\var{\mathrm{var}}
\def\Cov{\mathrm{Cov}}
\def\Tr{\mathrm{Tr}}
\def\rank{\mathrm{rank}}
\def\alphabar{\overline{\alpha}}
\def\etabar{\overline{\eta}}
\def\gammabar{\overline{\gamma}}
\def\gammatil{\tilde{\gamma}}
\def\PL2{\stackrel{PL(2)}{=}}


\def\tm{t\! - \!}
\def\tp{t\! + \!}
\def\km{k\! - \!}
\def\kp{k\! + \!}
\def\lp{\ell\! + \!}
\def\lm{\ell\! - \!}
\def\Lm{L\! - \!}
\def\ip{i\! + \!}
\def\im{i\! - \!}

\def\Xset{{\cal X}}

\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\abf}{\mathbf{a}}
\newcommand{\bbf}{\mathbf{b}}
\newcommand{\cbf}{\mathbf{c}}
\newcommand{\cbfhat}{\widehat{\mathbf{c}}}
\newcommand{\dbf}{\mathbf{d}}
\newcommand{\ebf}{\mathbf{e}}
\newcommand{\fbf}{\mathbf{f}}
\newcommand{\gbf}{\mathbf{g}}
\newcommand{\hbf}{\mathbf{h}}
\newcommand{\pbf}{\mathbf{p}}
\newcommand{\pbfhat}{\widehat{\mathbf{p}}}
\newcommand{\qbf}{\mathbf{q}}
\newcommand{\qbfhat}{\widehat{\mathbf{q}}}
\newcommand{\rbf}{\mathbf{r}}
\newcommand{\rbfhat}{\widehat{\mathbf{r}}}
\newcommand{\rbftil}{\tilde{\mathbf{r}}}
\newcommand{\sbf}{\mathbf{s}}
\newcommand{\sbfbar}{\overline{\mathbf{s}}}
\newcommand{\sbfhat}{\widehat{\mathbf{s}}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\ubfhat}{\widehat{\mathbf{u}}}
\newcommand{\ubftil}{\tilde{\mathbf{u}}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\vbfhat}{\widehat{\mathbf{v}}}
\newcommand{\wbfhat}{\wh{\wbf}}
\newcommand{\xbf}{\bm{x}}
\newcommand{\xbfbar}{\wb{\xbf}}
\newcommand{\xbfhat}{\wh{\xbf}}
\newcommand{\xbftil}{\wt{\mathbf{x}}}
\newcommand{\ybfbar}{\overline{\ybf}}
\newcommand{\ybftil}{\wt{\ybf}}
\newcommand{\zbf}{\mathbf{z}}
\newcommand{\zbfbar}{\overline{\mathbf{z}}}
\newcommand{\zbfhat}{\widehat{\mathbf{z}}}
\newcommand{\Abf}{\mathbf{A}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\Bbfhat}{\wh{\mathbf{B}}}
\newcommand{\Cbf}{\mathbf{C}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\Gbf}{\mathbf{G}}
\newcommand{\Gabf}{\mathbf{\Gamma}}
\newcommand{\Hbf}{\mathbf{H}}
\newcommand{\Hbar}{\overline{H}}
\newcommand{\Ibf}{\mathbf{I}}
\newcommand{\Jbf}{\mathbf{J}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Kbf}{\mathbf{K}}
\newcommand{\Lbf}{\mathbf{L}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Phat}{\wh{P}}
\newcommand{\Qbf}{\mathbf{Q}}
\newcommand{\Rbf}{\mathbf{R}}
\newcommand{\Rhat}{\wh{R}}
\newcommand{\Sbf}{\mathbf{S}}
\newcommand{\Ubf}{\mathbf{U}}
\newcommand{\Ubftil}{\wt{\mathbf{U}}}
\newcommand{\Ubfbar}{\overline{\mathbf{U}}}
\newcommand{\Vbf}{\mathbf{V}}
\newcommand{\Vbftil}{\wt{\mathbf{V}}}
\newcommand{\Vbfbar}{\overline{\mathbf{V}}}
\newcommand{\Wbf}{\mathbf{W}}
\newcommand{\What}{\wh{W}}
\newcommand{\Xhat}{\wh{X}}
\newcommand{\Xbf}{\mathbf{X}}
\newcommand{\Ybf}{\mathbf{Y}}
\newcommand{\Zbf}{\mathbf{Z}}
\newcommand{\Zhat}{\wh{Z}}
\newcommand{\Yhat}{\wh{Y}}
\newcommand{\Zbfhat}{\wh{\mathbf{Z}}}
\newcommand{\inner}[1]{\langle{#1}\rangle}
\def\alphabf{{\boldsymbol \alpha}}
\def\betabf{{\boldsymbol \beta}}
\def\mubf{{\boldsymbol \mu}}
\def\gammabf{{\boldsymbol \gamma}}
\def\Gammabf{{\boldsymbol \Gamma}}
\def\lambdabf{{\boldsymbol \lambda}}
\def\Lambdabf{{\boldsymbol \Lambda}}
\def\lambdabar{\overline{\lambda}}
\def\Lambdabar{\overline{\Lambda}}
\def\lambdabfbar{\overline{\lambdabf}}
\def\Lambdabfbar{\overline{\Lambdabf}}
\def\gammabfbar{\overline{\gammabf}}
\def\Gammabfbar{\overline{\Gammabf}}
\def\thetabfbar{\overline{\thetabf}}
\def\Thetabfbar{\overline{\Thetabf}}
\def\omegabfbar{\overline{\omegabf}}
\def\Omegabfbar{\overline{\Omegabf}}
% \newcommand{\Lambdabf}{\mathbf{\lambda}}
\def\Sigmabf{{\boldsymbol \Sigma}}
\def\etabf{{\boldsymbol \eta}}
\def\nubf{{\boldsymbol \nu}}
\def\xibf{{\boldsymbol \xi}}
\def\Xibf{{\boldsymbol \Xi}}
\def\taubf{{\boldsymbol \tau}}
\def\taubar{{\overline{\tau}}}
\def\taubfbar{{\overline{\boldsymbol \tau}}}
\def\taubfhat{{\wh{\boldsymbol \tau}}}
\def\varphibf{{\boldsymbol \varphi}}
\def\phihat{{\wh{\phi}}}
\def\Psibf{\boldsymbol{\Psi}}
\def\psibf{\boldsymbol{\psi}}
\def\muhat{{\wh{\mu}}}
\newcommand{\thetabar}{{\overline{\theta}}}
\newcommand{\thetabf}{{\bm{\theta}}}
\newcommand{\Thetabf}{{\bm{\Theta}}}
\newcommand{\omegabf}{{\bm{\omaga}}}
\newcommand{\Omegabf}{{\bm{\Omega}}}
\newcommand{\phibf}{{\bm{\phi}}}
\newcommand{\thetahat}{{\wh{\theta}}}
\newcommand{\mubar}{\overline{\mu}}
\newcommand{\muavg}{\mu}
\newcommand{\sigbf}{\bm{\sigma}}
\newcommand{\etal}{\emph{et al.}}
\def\Pset{{\mathcal P}}
\newcommand{\bigCond}[2]{\bigl({#1} \!\bigm\vert\! {#2} \bigr)}
\newcommand{\BigCond}[2]{\Bigl({#1} \!\Bigm\vert\! {#2} \Bigr)}
\newcommand{\indic}[1]{\mathbbm{1}_{ \{ {#1} \} }}



\newcommand{\MAP}{_{\text{\sf MAP}}}
\newcommand{\MMSE}{_{\text{\sf MMSE}}}
\newcommand{\opt}{_{\text{\sf opt}}}
\newcommand{\tran}{^{\text{\sf T}}}
\newcommand{\herm}{^{\text{\sf H}}}
\newcommand{\fz}{f_z}
\newcommand{\fzi}{f_{z_i}}
\newcommand{\fx}{f_x}
\newcommand{\fxj}{f_{x_j}}
\newcommand{\Zz}{Z_z}
\newcommand{\Zx}{Z_x}
\newcommand{\ZzT}{Z_{z,T}}
\newcommand{\ZxT}{Z_{x,T}}
\newcommand{\pdf}{p}
\newcommand{\ALG}{ADMM-GAMP\xspace}
\newcommand{\defn}{:=}
\newcommand{\const}{\text{const}}
\def\Hmax{H_{\rm max}}
\def\gt{\wt{g}}

\def\negSpace{\hspace{-0.15in}}
\def\eqd{\stackrel{d}{=}}
\def\PLeq{\stackrel{PL(2)}{=}}
\def\Norm{{\mathcal N}}
\def\Range{\mathrm{Range}}
\def\Diag{\mathrm{Diag}}
\def\alphabar{\overline{\alpha}}
\def\xbft{\wt{\xbf}}
\def\zbft{\wt{\mathbf{z}}}
\def\Ecal{{\mathcal E}}
\def\Kit{K_{\text{\sf it}}}

\newcommand*\dif{\mathop{}\!\mathrm{d}} % differential in integrals
\newcommand{\Hessian}[1]{\boldsymbol{\mathcal{H}}_{#1}} % differential in integrals
\newcommand{\vmult}{.}
\newcommand{\vdiv}{./}
\newcommand{\bkt}[1]{{\left< #1 \right>}}
\newcommand{\bktAuto}[1]{{\left\langle #1 \right\rangle}} % Auto for automatically sized
\def\Gset{\mathfrak{G}}
\def\Gsetbar{\overline{\mathfrak{G}}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Parthe's Macros%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\pp}[1]{\textcolor{magenta}{PP: #1}}
\providecommand{\orange}[1]{\textcolor{orange}{#1}}
\providecommand{\black}[1]{\textcolor{black}{#1}}
\providecommand{\red}[1]{\textcolor{red}{#1}}
\providecommand{\blue}[1]{\textcolor{blue}{#1}}
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\magenta}[1]{\textcolor{magenta}{#1}}
\providecommand{\gray}[1]{\textcolor{black!50}{#1}}
\providecommand{\old}[1]{ }
\providecommand{\aur}{\ {\rm and}\ }
\providecommand{\mmse}{\text{\sf mmse}}
\providecommand{\map}{\text{\sf map}}
\providecommand{\mest}{\text{\sf m-est}}
\providecommand{\Var}{{\rm Var}}
\providecommand{\mc}{\mathcal}
\providecommand{\ie}{{\rm i.e.}}
\providecommand{\T}{^\top}
\providecommand{\wb}{\overline}
\providecommand{\wt}{\widetilde}
\providecommand{\wh}{\widehat}
\newcommand{\norm}[1]{\left\|#1\right\|}
\providecommand{\Real}{\mathbb{R}}



\providecommand{\a}{\bm{a}}
\providecommand{\b}{\bm{b}}
\providecommand{\bmc}{\bm{c}} % This is a special accented character like Ca\c{c}mak (pronounced Chuk Muck)
\providecommand{\d}{\bm{d}}
\providecommand{\e}{\bm{e}}
\providecommand{\f}{\bm{f}}
\providecommand{\g}{\bm{g}}
\providecommand{\h}{\bm{h}}
\providecommand{\i}{\bm{i}}
\providecommand{\j}{\bm{j}}
\providecommand{\k}{\bm{k}}
\providecommand{\l}{\bm{l}}
\providecommand{\m}{\bm{m}}
\providecommand{\n}{\bm{n}}
\providecommand{\o}{\bm{o}}
\providecommand{\p}{\mathbf{p}}
\providecommand{\q}{\mathbf{q}}
\renewcommand{\r}{\bm{r}}
\providecommand{\s}{\bm{s}}
\providecommand{\t}{\bm{t}}
\providecommand{\u}{\bm{u}}
\providecommand{\v}{\bm{v}}
\providecommand{\w}{\mathbf{w}}
\providecommand{\x}{\bm{x}}
\providecommand{\y}{\bm{y}}
\providecommand{\z}{\mathbf{z}}


\providecommand{\A}{\bm{A}}
\providecommand{\G}{\bm{G}}
\providecommand{\I}{\bm{I}}
\providecommand{\S}{\bm{S}}
\providecommand{\U}{\bm{U}}
\providecommand{\V}{\bm{V}}
\providecommand{\W}{\bm{W}}
\providecommand{\X}{\bm{X}}
\providecommand{\Y}{\bm{Y}}
\providecommand{\Z}{\bm{Z}}
\providecommand{\M}{\bm{M}}
\providecommand{\K}{\bm{K}}
%% Boldfaced lowercase and UPPERCASE
\providecommand{\abf}{\mathbf{a}}
\providecommand{\bbf}{\mathbf{b}}
\providecommand{\cbf}{\mathbf{c}}
\providecommand{\dbf}{\mathbf{d}}
\providecommand{\ebf}{\mathbf{e}}
\providecommand{\fbf}{\mathbf{f}}
\providecommand{\gbf}{\mathbf{g}}
\providecommand{\hbf}{\mathbf{h}}
\providecommand{\ibf}{\mathbf{i}}
\providecommand{\jbf}{\mathbf{j}}
\providecommand{\kbf}{\mathbf{k}}
\providecommand{\lbf}{\mathbf{l}}
%\providecommand{\mbf}{\mathbf{m}}
\providecommand{\nbf}{\mathbf{n}}
\providecommand{\obf}{\mathbf{o}}
\providecommand{\pbf}{\mathbf{p}}
\providecommand{\qbf}{\mathbf{q}}
\providecommand{\rbf}{\mathbf{r}}
\providecommand{\sbf}{\mathbf{s}}
\providecommand{\tbf}{\mathbf{t}}
\providecommand{\ubf}{\mathbf{u}}
\providecommand{\vbf}{\mathbf{v}}
\providecommand{\wbf}{\bm{w}}
\providecommand{\xbf}{\bm{x}}
\providecommand{\ybf}{\bm{y}}
\providecommand{\zbf}{\mathbf{z}}
\providecommand{\Abf}{\mathbf{A}}
\providecommand{\Bbf}{\mathbf{B}}
\providecommand{\Cbf}{\mathbf{C}}
\providecommand{\Dbf}{\mathbf{D}}
\providecommand{\Ebf}{\mathbf{E}}
\providecommand{\Fbf}{\mathbf{F}}
\providecommand{\Gbf}{\mathbf{G}}
\providecommand{\Hbf}{\mathbf{H}}
\providecommand{\Ibf}{\mathbf{I}}
\providecommand{\Jbf}{\mathbf{J}}
\providecommand{\Kbf}{\mathbf{K}}
\providecommand{\Lbf}{\mathbf{L}}
\providecommand{\Mbf}{\mathbf{M}}
\providecommand{\Nbf}{\mathbf{N}}
\providecommand{\Obf}{\mathbf{O}}
\providecommand{\Pbf}{\mathbf{P}}
\providecommand{\Qbf}{\mathbf{Q}}
\providecommand{\Rbf}{\mathbf{R}}
\providecommand{\Sbf}{\mathbf{S}}
\providecommand{\Tbf}{\mathbf{T}}
\providecommand{\Ubf}{\mathbf{U}}
\providecommand{\Vbf}{\mathbf{V}}
\providecommand{\Wbf}{\mathbf{W}}
\providecommand{\Xbf}{\mathbf{X}}
\providecommand{\Ybf}{\mathbf{Y}}
\providecommand{\Zbf}{\mathbf{Z}}

\providecommand{\bfa}{\mathbf{a}}
\providecommand{\bfb}{\mathbf{b}}
\providecommand{\bfc}{\mathbf{c}}
\providecommand{\bfd}{\mathbf{d}}
\providecommand{\bfe}{\mathbf{e}}
\providecommand{\bff}{\mathbf{f}}
\providecommand{\bfg}{\mathbf{g}}
\providecommand{\bfh}{\mathbf{h}}
\providecommand{\bfi}{\mathbf{i}}
\providecommand{\bfj}{\mathbf{j}}
\providecommand{\bfk}{\mathbf{k}}
\providecommand{\bfl}{\mathbf{l}}
\providecommand{\bfm}{\mathbf{m}}
\providecommand{\bfn}{\mathbf{n}}
\providecommand{\bfo}{\mathbf{o}}
\providecommand{\bfp}{\mathbf{p}}
\providecommand{\bfq}{\mathbf{q}}
\providecommand{\bfr}{\mathbf{r}}
\providecommand{\bfs}{\mathbf{s}}
\providecommand{\bft}{\mathbf{t}}
\providecommand{\bfu}{\mathbf{u}}
\providecommand{\bfv}{\mathbf{v}}
\providecommand{\bfw}{\mathbf{w}}
\providecommand{\bfx}{\mathbf{x}}
\providecommand{\bfy}{\mathbf{y}}
\providecommand{\bfz}{\mathbf{z}}
\providecommand{\bfA}{\mathbf{A}}
\providecommand{\bfB}{\mathbf{B}}
\providecommand{\bfC}{\mathbf{C}}
\providecommand{\bfD}{\mathbf{D}}
\providecommand{\bfE}{\mathbf{E}}
\providecommand{\bfF}{\mathbf{F}}
\providecommand{\bfG}{\mathbf{G}}
\providecommand{\bfH}{\mathbf{H}}
\providecommand{\bfI}{\mathbf{I}}
\providecommand{\bfJ}{\mathbf{J}}
\providecommand{\bfK}{\mathbf{K}}
\providecommand{\bfL}{\mathbf{L}}
\providecommand{\bfM}{\mathbf{M}}
\providecommand{\bfN}{\mathbf{N}}
\providecommand{\bfO}{\mathbf{O}}
\providecommand{\bfP}{\mathbf{P}}
\providecommand{\bfQ}{\mathbf{Q}}
\providecommand{\bfR}{\mathbf{R}}
\providecommand{\bfS}{\mathbf{S}}
\providecommand{\bfT}{\mathbf{T}}
\providecommand{\bfU}{\mathbf{U}}
\providecommand{\bfV}{\mathbf{V}}
\providecommand{\bfW}{\mathbf{W}}
\providecommand{\bfX}{\mathbf{X}}
\providecommand{\bfY}{\mathbf{Y}}
\providecommand{\bfZ}{\mathbf{Z}}


\providecommand{\phibf}{\mbf{\phi}}

%% CALIGRAPHIC UPPERCASE
\providecommand{\mcA}{\mathcal{A}}
\providecommand{\mcB}{\mathcal{B}}
\providecommand{\mcC}{\mathcal{C}}
\providecommand{\mcD}{\mathcal{D}}
\providecommand{\mcE}{\mathcal{E}}
\providecommand{\mcF}{\mathcal{F}}
\providecommand{\mcG}{\mathcal{G}}
\providecommand{\mcH}{\mathcal{H}}
\providecommand{\mcI}{\mathcal{I}}
\providecommand{\mcJ}{\mathcal{J}}
\providecommand{\mcK}{\mathcal{K}}
\providecommand{\mcL}{\mathcal{L}}
\providecommand{\mcM}{\mathcal{M}}
\providecommand{\mcN}{\mathcal{N}}
\providecommand{\mcO}{\mathcal{O}}
\providecommand{\mcP}{\mathcal{P}}
\providecommand{\mcQ}{\mathcal{Q}}
\providecommand{\mcR}{\mathcal{R}}
\providecommand{\mcS}{\mathcal{S}}
\providecommand{\mcT}{\mathcal{T}}
\providecommand{\mcU}{\mathcal{U}}
\providecommand{\mcV}{\mathcal{V}}
\providecommand{\mcW}{\mathcal{W}}
\providecommand{\mcX}{\mathcal{X}}
\providecommand{\mcY}{\mathcal{Y}}
\providecommand{\mcZ}{\mathcal{Z}}
\newcommand\blankfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\providecommand{\indic}[1]{\mathbbm{1}_{ \{ {#1} \} }}
\providecommand{\bs}[1]{\boldsymbol{#1}}
\providecommand{\wbar}[1]{\overline{{#1}}}
\providecommand{\ignore}[1]{}
\renewcommand{\r}{\bm{r}}
\renewcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\Eta}{H}
\renewcommand{\R}{\bm{R}}
\renewcommand{\a}{\bm{a}}
\renewcommand{\Z}{\bm{Z}}
\renewcommand{\S}{\bm{S}}
\renewcommand{\Q}{\bm{Q}}
\renewcommand{\P}{\bm{P}}
\renewcommand{\H}{\bm{H}}
\newcommand{\kappabf}{\bm{\kappa}}

\newcommand{\Qtil}{\wt{Q}}
\newcommand{\tl}[1]{\widetilde{{#1}}}
\newcommand{\convd}{\stackrel{d}{\rightarrow}}

\providecommand{\wh}[1]{\widehat{{#1}}}
% \newcommand{\Exp}{\mathbb{E}}
% \newcommand{\C}{\mathbb{C}}
% \newcommand{\mc}[1]{\mathcal{#1}}
% \newcommand{\Norm}{\mc{N}}
\newcommand{\CNorm}{\mc{N}_{\mathbb{C}}}
\newcommand{\subsf}{\sf \scriptscriptstyle}


